Predicted masses of Galactic Cepheids in the Gaia Data Release 2

On the basis of recently computed nonlinear convective pulsation models of Galactic Cepheids, spanning wide ranges of input stellar parameters, we derive theoretical mass-dependent Period-Wesenheit relations in the Gaia bands, namely $G$, $G_{BP}$ and $G_{RP}$, that are found to be almost independent of the assumed efficiency of super-adiabatic convection. The application to a selected sub-sample of Gaia Data Release 2 Galactic Cepheids database allows us to derive mass-dependent estimates of their individual distances. By imposing their match with the astrometric values inferred from Gaia, we are able to evaluate the individual mass of each pulsator. The inferred mass distribution is peaked around 5.6$M_{\odot}$ and 5.4$M_{\odot}$ for the F and FO pulsators, respectively. If the estimated Gaia parallax offset $<\Delta\varpi>$=0.046 mas is applied to Gaia parallaxes before imposing their coincidence with the theoretical ones, the inferred mass distribution is found to shift towards lower masses, namely $\sim$5.2$M_{\odot}$ and 5.1$M_{\odot}$ for the F and FO pulsators, respectively. The comparison with independent evaluations of the stellar masses, for a subset of binary Cepheids in our sample, seems to support the predictive capability of current theoretical scenario. By forcing the coincidence of our mass determinations with these literature values we derive an independent estimate of the mean offset to be applied to Gaia DR2 parallaxes, $<\Delta\varpi>$=0.053 $\pm$ 0.029 mas, slightly higher but in agreement within the errors with Riess2018 value.

==> tab_all_F_FO_1p5.tex <==
\begin{table*}
\caption{\label{mass_F_1.5} The individual masses estimated from the theoretical PWM relations combined with Gaia DR2 parallaxes, for F-mode GCC in the selected sample. This table is available in its entirety in machine-readable form.}
\centering
\begin{tabular}{cccccccccccc}
\hline\hline
\textsl{Gaia} DR2 Source Id & P[d] & $G$[mag] & $G_{BP}$[mag] & $G_{RP}$[mag] & $\varpi$[mas] & $\sigma$$\varpi$[mas] & \msun & $\sigma$\msun & \msun{corr} &  $\sigma$\msun{corr}\\
\hline
Gaia DR2 source Id & Mode & P[d] & G[mag] & G_BP[mag] & G_RP[mag] & Plx[mas] & sigma_plx[mas] & M/Ms & sigmaM/Ms & M/Mscorr & sigmaM/Mscorr \\
1857884212378132096 & F & 4.43546 & 5.46 & 5.77 & 5.07 & 1.674 & 0.089 & 4.2 & 0.5 & 4.0 & 0.5 \\
4066429066901946368 & F & 5.05787 & 6.82 & 7.37 & 6.23 & 1.119 & 0.053 & 5.2 & 0.6 & 4.8 & 0.5 \\
5235910694044165760 & F & 3.08613 & 8.70 & 9.22 & 8.06 & 0.681 & 0.032 & 4.1 & 0.5 & 3.6 & 0.4 \\
279382060625871360 & F & 3.29487 & 7.19 & 7.81 & 6.48 & 1.272 & 0.035 & 6.2 & 0.5 & 5.7 & 0.4 \\
5824464493705913472 & F & 3.38932 & 6.44 & 6.86 & 5.91 & 1.475 & 0.037 & 4.5 & 0.3 & 4.3 & 0.3 \\
5932997939411720960 & F & 3.45291 & 9.79 & 10.63 & 8.92 & 0.547 & 0.036 & 5.5 & 0.8 & 4.7 & 0.7 \\
5351721738384434048 & F & 3.68221 & 8.08 & 8.45 & 7.59 & 0.561 & 0.037 & 5.4 & 0.8 & 4.6 & 0.7 \\
465719182408723072 & F & 3.83288 & 10.43 & 11.14 & 9.64 & 0.307 & 0.028 & 6.1 & 1.2 & 4.6 & 0.9 \\
6059635702888301952 & F & 3.83834 & 7.99 & 8.43 & 7.42 & 0.621 & 0.038 & 6.1 & 0.8 & 5.3 & 0.7 \\
2166861170366710272 & F & 4.04921 & 10.29 & 11.11 & 9.41 & 0.528 & 0.028 & 3.1 & 0.4 & 2.6 & 0.3 \\
422923956470923008 & F & 4.07117 & 9.54 & 10.14 & 8.83 & 0.399 & 0.030 & 5.6 & 0.9 & 4.5 & 0.7 \\
3027940437469882880 & F & 4.25689 & 9.32 & 9.95 & 8.59 & 0.492 & 0.040 & 4.7 & 0.8 & 3.9 & 0.7 \\
5338024572321721216 & F & 4.26618 & 9.44 & 9.99 & 8.79 & 0.374 & 0.027 & 5.5 & 0.9 & 4.3 & 0.7 \\
2014609252631258496 & F & 4.27863 & 11.57 & 12.60 & 10.58 & 0.390 & 0.027 & 2.9 & 0.4 & 2.3 & 0.4 \\
1977074811892425600 & F & 4.32355 & 8.96 & 9.40 & 8.39 & 0.403 & 0.034 & 5.2 & 0.9 & 4.2 & 0.8 \\
2060021625508894592 & F & 4.36470 & 9.49 & 10.10 & 8.77 & 0.399 & 0.028 & 5.6 & 0.9 & 4.5 & 0.7 \\
6055722403534963840 & F & 4.42452 & 9.46 & 10.21 & 8.65 & 0.446 & 0.031 & 6.9 & 1.1 & 5.7 & 0.9 \\
426881614218441600 & F & 4.50162 & 9.55 & 10.21 & 8.79 & 0.403 & 0.030 & 6.0 & 1.0 & 4.8 & 0.8 \\
4054440301294394624 & F & 4.52781 & 7.55 & 8.14 & 6.92 & 0.920 & 0.047 & 5.1 & 0.6 & 4.6 & 0.5 \\
5521459979795304320 & F & 4.63985 & 7.71 & 8.26 & 7.05 & 0.852 & 0.035 & 4.9 & 0.5 & 4.4 & 0.4 \\
5338438297925480320 & F & 4.67767 & 9.41 & 9.97 & 8.73 & 0.375 & 0.026 & 5.6 & 0.9 & 4.4 & 0.7 \\
3046774762417915136 & F & 4.67830 & 7.83 & 8.33 & 7.20 & 0.616 & 0.047 & 7.3 & 1.2 & 6.3 & 1.0 \\
6060173364061645696 & F & 4.68971 & 6.36 & 6.80 & 5.79 & 1.021 & 0.045 & 8.5 & 0.9 & 7.7 & 0.8 \\
1960750328384177408 & F & 4.86438 & 8.67 & 9.19 & 8.03 & 0.435 & 0.028 & 6.8 & 1.0 & 5.5 & 0.8 \\
2078709577944648192 & F & 4.92549 & 8.90 & 9.42 & 8.26 & 0.413 & 0.023 & 6.1 & 0.8 & 4.9 & 0.6 \\
5258574068220187648 & F & 4.93255 & 10.24 & 10.94 & 9.46 & 0.365 & 0.032 & 3.9 & 0.7 & 3.1 & 0.6 \\
2055122987639665664 & F & 4.95045 & 12.27 & 13.38 & 11.21 & 0.339 & 0.033 & 2.3 & 0.5 & 1.7 & 0.4 \\
270272675510149504 & F & 4.97249 & 9.12 & 9.99 & 8.23 & 0.521 & 0.038 & 8.9 & 1.4 & 7.5 & 1.2 \\
2003938801532007808 & F & 4.98330 & 8.61 & 9.15 & 7.94 & 0.437 & 0.035 & 7.7 & 1.3 & 6.2 & 1.1 \\
2011315528113463808 & F & 4.99754 & 10.50 & 11.42 & 9.58 & 0.355 & 0.026 & 6.1 & 1.0 & 4.8 & 0.8 \\
473293889810320128 & F & 5.06643 & 10.00 & 11.16 & 8.95 & 0.716 & 0.031 & 4.5 & 0.5 & 3.9 & 0.4 \\
5871738271033526016 & F & 5.07890 & 7.43 & 7.89 & 6.85 & 0.841 & 0.034 & 4.4 & 0.4 & 4.0 & 0.4 \\
2166303099490547072 & F & 5.09955 & 10.53 & 11.69 & 9.46 & 0.528 & 0.027 & 5.2 & 0.6 & 4.4 & 0.5 \\
4080122796947250176 & F & 5.15424 & 7.25 & 7.83 & 6.58 & 0.986 & 0.047 & 5.3 & 0.6 & 4.9 & 0.5 \\
4085919765884068736 & F & 6.63703 & 6.63 & 7.21 & 5.93 & 1.248 & 0.041 & 5.0 & 0.4 & 4.6 & 0.4 \\
1827869808377481216 & F & 5.19725 & 10.03 & 10.96 & 9.09 & 0.419 & 0.034 & 6.8 & 1.2 & 5.5 & 1.0 \\
5254295559276699392 & F & 5.20456 & 9.06 & 9.56 & 8.44 & 0.374 & 0.028 & 5.6 & 0.9 & 4.4 & 0.7 \\
1968971582984827136 & F & 5.25760 & 8.88 & 9.91 & 7.90 & 0.896 & 0.027 & 5.4 & 0.4 & 4.9 & 0.4 \\
6053622679932061056 & F & 5.26567 & 9.01 & 9.91 & 8.12 & 0.783 & 0.045 & 4.2 & 0.5 & 3.8 & 0.5 \\
4147381366335558784 & F & 5.30141 & 9.96 & 11.03 & 8.94 & 0.670 & 0.040 & 4.1 & 0.5 & 3.6 & 0.5 \\
5334506135119058304 & F & 5.30996 & 8.49 & 9.08 & 7.79 & 0.549 & 0.032 & 5.8 & 0.8 & 4.9 & 0.6 \\
1960981328902089088 & F & 5.33166 & 8.57 & 9.13 & 7.90 & 0.509 & 0.031 & 5.7 & 0.8 & 4.7 & 0.6 \\
458239995077788544 & F & 5.36511 & 10.46 & 11.49 & 9.51 & 0.366 & 0.035 & 7.1 & 1.4 & 5.6 & 1.1 \\
4190143160245024256 & F & 5.37668 & 7.54 & 8.03 & 6.92 & 0.738 & 0.052 & 5.6 & 0.9 & 4.9 & 0.8 \\
2010285491880986112 & F & 5.44090 & 9.28 & 9.96 & 8.51 & 0.413 & 0.032 & 6.5 & 1.1 & 5.2 & 0.9 \\
5891675303053080704 & F & 5.49457 & 6.55 & 7.11 & 5.93 & 1.340 & 0.045 & 4.6 & 0.4 & 4.3 & 0.4 \\
459035766618689280 & F & 5.53070 & 10.37 & 11.47 & 9.37 & 0.394 & 0.035 & 8.1 & 1.5 & 6.4 & 1.2 \\
5539107450645759232 & F & 5.56408 & 10.59 & 11.47 & 9.75 & 0.258 & 0.025 & 7.8 & 1.6 & 5.6 & 1.1 \\
422226488141991296 & F & 5.80901 & 8.78 & 9.37 & 8.08 & 0.359 & 0.033 & 9.7 & 1.9 & 7.5 & 1.5 \\
5327836325732931840 & F & 5.85935 & 9.21 & 9.96 & 8.39 & 0.407 & 0.029 & 8.2 & 1.3 & 6.6 & 1.0 \\
5436296928693979392 & F & 5.89839 & 9.12 & 9.52 & 8.58 & 0.292 & 0.029 & 5.7 & 1.2 & 4.2 & 0.9 \\
2055014277739104896 & F & 5.95590 & 8.91 & 9.76 & 8.02 & 0.697 & 0.039 & 4.8 & 0.6 & 4.2 & 0.5 \\
4092905375639902464 & F & 6.74522 & 6.35 & 7.01 & 5.62 & 1.460 & 0.045 & 5.6 & 0.5 & 5.2 & 0.4 \\
4312361436842603520 & F & 6.11423 & 7.66 & 8.44 & 6.84 & 0.930 & 0.057 & 6.6 & 0.9 & 5.9 & 0.8 \\
6059764002146656128 & F & 6.22040 & 8.07 & 8.64 & 7.38 & 0.524 & 0.046 & 7.8 & 1.5 & 6.5 & 1.2 \\
2008504454839717120 & F & 6.23397 & 9.00 & 9.92 & 8.08 & 0.679 & 0.030 & 5.4 & 0.6 & 4.7 & 0.5 \\
525136962570940160 & F & 6.27279 & 10.23 & 11.24 & 9.28 & 0.374 & 0.028 & 6.9 & 1.1 & 5.5 & 0.9 \\
2015820463470505600 & F & 6.29664 & 9.24 & 10.22 & 8.28 & 0.588 & 0.032 & 6.8 & 0.8 & 5.8 & 0.7 \\
5823134325151372032 & F & 6.31663 & 6.22 & 6.59 & 5.63 & 1.075 & 0.030 & 5.8 & 0.4 & 5.4 & 0.4 \\
2027263738130844288 & F & 6.32059 & 8.23 & 9.14 & 7.30 & 0.841 & 0.039 & 7.1 & 0.8 & 6.4 & 0.7 \\
4096979650282842112 & F & 6.42429 & 8.41 & 9.08 & 7.59 & 0.702 & 0.059 & 4.5 & 0.8 & 3.9 & 0.7 \\
5312196047720402048 & F & 6.45380 & 11.06 & 12.07 & 10.08 & 0.275 & 0.026 & 6.2 & 1.2 & 4.5 & 0.9 \\
5868480143187802240 & F & 6.45975 & 8.08 & 8.71 & 7.34 & 0.557 & 0.039 & 7.9 & 1.2 & 6.7 & 1.0 \\
174489098011145216 & F & 6.46466 & 7.05 & 7.73 & 6.27 & 1.042 & 0.064 & 6.8 & 0.9 & 6.2 & 0.9 \\
5541507237862358912 & F & 6.66423 & 7.71 & 8.14 & 7.16 & 0.568 & 0.030 & 5.3 & 0.6 & 4.5 & 0.5 \\
5302258008774271488 & F & 6.69695 & 7.11 & 7.60 & 6.50 & 0.760 & 0.023 & 6.2 & 0.5 & 5.5 & 0.4 \\
6054829806275577216 & F & 6.73287 & 6.30 & 6.81 & 5.68 & 1.140 & 0.028 & 6.2 & 0.4 & 5.7 & 0.4 \\
4204653587029046400 & F & 6.80601 & 7.34 & 8.02 & 6.57 & 0.944 & 0.048 & 5.9 & 0.7 & 5.3 & 0.6 \\
5324034867356093056 & F & 6.92436 & 7.22 & 7.93 & 6.44 & 1.007 & 0.037 & 6.1 & 0.6 & 5.5 & 0.5 \\
4057701830728920064 & F & 7.01753 & 4.21 & 4.75 & 3.70 & 3.431 & 0.202 & 3.8 & 0.5 & 3.7 & 0.5 \\
5877533315817003648 & F & 7.06626 & 6.42 & 6.96 & 5.77 & 1.015 & 0.032 & 7.4 & 0.6 & 6.7 & 0.6 \\
5309174967720762496 & F & 7.13431 & 9.69 & 10.51 & 8.83 & 0.312 & 0.029 & 8.9 & 1.8 & 6.7 & 1.3 \\
5257664497238811776 & F & 7.19619 & 8.95 & 9.58 & 8.22 & 0.355 & 0.030 & 7.8 & 1.4 & 6.1 & 1.1 \\
4307944836090489600 & F & 7.23996 & 9.35 & 10.33 & 8.39 & 0.554 & 0.055 & 5.9 & 1.3 & 5.0 & 1.1 \\
2165771172070496512 & F & 7.25140 & 9.95 & 10.88 & 9.00 & 0.387 & 0.028 & 6.4 & 1.0 & 5.1 & 0.8 \\
5855468247702904704 & F & 7.51028 & 6.10 & 6.55 & 5.55 & 1.000 & 0.029 & 6.9 & 0.5 & 6.3 & 0.5 \\
5337191279923824384 & F & 7.53200 & 7.80 & 8.35 & 7.14 & 0.704 & 0.030 & 4.0 & 0.4 & 3.5 & 0.4 \\
5339394082770287232 & F & 7.72081 & 6.61 & 7.08 & 6.01 & 0.796 & 0.035 & 7.5 & 0.8 & 6.7 & 0.7 \\
2016028168089215488 & F & 7.80112 & 10.08 & 11.04 & 9.12 & 0.383 & 0.031 & 5.7 & 1.0 & 4.5 & 0.8 \\
2030063919381336832 & F & 7.81823 & 9.37 & 10.16 & 8.51 & 0.400 & 0.032 & 6.3 & 1.1 & 5.1 & 0.9 \\
1873112207907294848 & F & 7.85582 & 9.05 & 9.82 & 8.20 & 0.446 & 0.028 & 6.4 & 0.9 & 5.2 & 0.7 \\
470361114339849472 & F & 7.91561 & 7.16 & 7.92 & 6.32 & 0.782 & 0.040 & 11.6 & 1.4 & 10.3 & 1.2 \\
1825621002188696448 & F & 7.99014 & 6.58 & 7.41 & 5.72 & 1.053 & 0.039 & 12.8 & 1.2 & 11.8 & 1.1 \\
428620663657823232 & F & 8.00066 & 8.51 & 9.23 & 7.71 & 0.422 & 0.034 & 10.0 & 1.7 & 8.1 & 1.4 \\
512524361613040640 & F & 8.37701 & 6.64 & 7.46 & 5.78 & 1.296 & 0.031 & 7.5 & 0.5 & 6.9 & 0.5 \\
5254097093074642944 & F & 9.19783 & 8.80 & 9.39 & 8.12 & 0.328 & 0.029 & 7.0 & 1.3 & 5.4 & 1.0 \\
4056026175045038464 & F & 9.31686 & 8.24 & 9.08 & 7.43 & 0.697 & 0.064 & 4.9 & 1.0 & 4.3 & 0.8 \\
5854560115494081024 & F & 9.46519 & 8.26 & 8.97 & 7.47 & 0.496 & 0.031 & 7.3 & 1.0 & 6.1 & 0.8 \\
4269036830424588800 & F & 9.48055 & 7.90 & 8.67 & 7.12 & 0.690 & 0.050 & 5.7 & 0.9 & 5.0 & 0.8 \\
5835124087174043136 & F & 9.75376 & 6.15 & 6.70 & 5.52 & 1.062 & 0.042 & 6.1 & 0.6 & 5.6 & 0.5 \\
2070224337474904064 & F & 10.14797 & 9.42 & 10.48 & 8.42 & 0.447 & 0.029 & 7.8 & 1.1 & 6.4 & 0.9 \\
506779550797525760 & F & 10.87727 & 8.84 & 9.58 & 8.04 & 0.330 & 0.031 & 9.1 & 1.8 & 6.9 & 1.4 \\
2007201567928631296 & F & 10.88439 & 8.04 & 8.70 & 7.29 & 0.458 & 0.038 & 7.9 & 1.4 & 6.5 & 1.2 \\
5871922507947292032 & F & 10.94947 & 7.47 & 8.03 & 6.79 & 0.537 & 0.042 & 7.1 & 1.2 & 6.0 & 1.0 \\
5313887130948758016 & F & 11.20064 & 8.88 & 9.83 & 7.95 & 0.391 & 0.032 & 11.3 & 2.0 & 9.0 & 1.6 \\
200708636406382720 & F & 11.62570 & 7.34 & 7.94 & 6.68 & 0.543 & 0.051 & 7.7 & 1.5 & 6.5 & 1.3 \\
5332375453374624640 & F & 11.63735 & 9.33 & 10.09 & 8.59 & 0.264 & 0.026 & 7.8 & 1.6 & 5.6 & 1.2 \\
5240441472232302848 & F & 12.43802 & 8.85 & 9.60 & 8.06 & 0.330 & 0.027 & 7.9 & 1.4 & 6.0 & 1.1 \\
5884729035255064064 & F & 12.63346 & 8.96 & 9.87 & 8.03 & 0.400 & 0.035 & 8.0 & 1.5 & 6.4 & 1.2 \\
4267397694768545920 & F & 13.75460 & 6.61 & 7.39 & 5.85 & 0.888 & 0.054 & 7.9 & 1.1 & 7.2 & 1.0 \\
5351331755370445056 & F & 14.10712 & 8.07 & 8.99 & 7.51 & 0.406 & 0.037 & 8.6 & 1.7 & 6.9 & 1.3 \\
6026412893938675712 & F & 6.06133 & 6.67 & 7.17 & 5.95 & 1.131 & 0.055 & 5.7 & 0.6 & 5.3 & 0.6 \\
2161786374436607616 & F & 14.71797 & 8.39 & 9.71 & 7.28 & 0.781 & 0.037 & 8.8 & 1.0 & 7.9 & 0.9 \\
2071433765909167232 & F & 15.11946 & 8.82 & 9.73 & 7.91 & 0.362 & 0.026 & 9.2 & 1.4 & 7.2 & 1.1 \\
1870258975238302208 & F & 16.39062 & 6.07 & 6.69 & 5.36 & 0.898 & 0.027 & 7.3 & 0.6 & 6.6 & 0.5 \\
5338036117182452096 & F & 16.65998 & 8.19 & 8.90 & 7.38 & 0.424 & 0.035 & 6.4 & 1.1 & 5.2 & 0.9 \\
2058374144759464064 & F & 17.07369 & 8.46 & 9.24 & 7.61 & 0.381 & 0.033 & 7.4 & 1.4 & 5.8 & 1.1 \\
4175017625462647168 & F & 17.12484 & 5.52 & 6.41 & 4.64 & 1.361 & 0.083 & 11.1 & 1.5 & 10.4 & 1.4 \\
5255254711361371520 & F & 18.17758 & 8.30 & 8.97 & 7.52 & 0.320 & 0.031 & 8.4 & 1.7 & 6.4 & 1.3 \\
5351161399785606016 & F & 18.87302 & 7.15 & 7.82 & 6.43 & 0.512 & 0.041 & 8.2 & 1.4 & 6.8 & 1.2 \\
1873250780732545920 & F & 20.14034 & 9.27 & 10.36 & 8.28 & 0.350 & 0.028 & 7.7 & 1.3 & 6.0 & 1.0 \\
5523162573544337408 & F & 20.49764 & 6.66 & 7.31 & 5.90 & 0.547 & 0.032 & 10.9 & 1.4 & 9.2 & 1.2 \\
5964193485048327808 & F & 28.86509 & 8.85 & 10.11 & 7.76 & 0.504 & 0.045 & 6.1 & 1.2 & 5.1 & 1.0 \\
5546476927338700416 & F & 41.46411 & 6.46 & 7.30 & 5.58 & 0.584 & 0.026 & 9.9 & 1.0 & 8.4 & 0.9 \\
5351436724362450304 & FO & 1.11936 & 11.09 & 11.62 & 10.41 & 0.389 & 0.030 & 3.3 & 0.7 & 2.4 & 0.5 \\
2164475809937299584 & FO & 1.76585 & 10.18 & 10.74 & 9.49 & 0.343 & 0.027 & 7.6 & 1.7 & 5.4 & 1.2 \\
5245796334347122944 & FO & 2.06344 & 8.09 & 8.53 & 7.54 & 0.858 & 0.026 & 3.5 & 0.4 & 3.0 & 0.3 \\
3398383973788673024 & FO & 2.10240 & 7.88 & 8.29 & 7.35 & 0.805 & 0.053 & 4.7 & 0.9 & 4.0 & 0.8 \\
2203988169026743936 & FO & 2.11413 & 7.51 & 8.05 & 6.84 & 1.133 & 0.033 & 5.6 & 0.6 & 5.0 & 0.5 \\
6057943520139661184 & FO & 2.30569 & 9.77 & 10.32 & 9.10 & 0.396 & 0.033 & 5.1 & 1.2 & 3.8 & 0.9 \\
5877460679352962048 & FO & 2.39812 & 7.29 & 7.73 & 6.70 & 0.995 & 0.040 & 5.7 & 0.7 & 5.0 & 0.6 \\
5824226655600824704 & FO & 2.42829 & 7.58 & 8.02 & 7.02 & 0.889 & 0.032 & 4.7 & 0.6 & 4.1 & 0.5 \\
1853025642297186688 & FO & 2.49930 & 5.62 & 5.93 & 5.20 & 1.706 & 0.055 & 4.7 & 0.5 & 4.4 & 0.5 \\
2007654601080023040 & FO & 2.80533 & 9.12 & 9.68 & 8.43 & 0.496 & 0.039 & 4.9 & 1.1 & 3.8 & 0.9 \\
429182376660681984 & FO & 2.84185 & 9.90 & 10.50 & 9.18 & 0.385 & 0.028 & 4.2 & 0.9 & 3.1 & 0.6 \\
4319599865468760832 & FO & 2.97303 & 10.15 & 11.24 & 9.14 & 0.571 & 0.038 & 6.2 & 1.2 & 5.0 & 1.0 \\
5258420858142702208 & FO & 3.03785 & 9.12 & 9.61 & 8.50 & 0.365 & 0.026 & 7.0 & 1.4 & 5.0 & 1.0 \\
2200929331984972672 & FO & 3.05313 & 10.87 & 11.74 & 9.96 & 0.317 & 0.027 & 5.5 & 1.4 & 3.8 & 0.9 \\
5848500161483878400 & FO & 3.06525 & 7.10 & 7.64 & 6.44 & 1.016 & 0.036 & 6.6 & 0.8 & 5.9 & 0.7 \\
5613541295473114496 & FO & 3.12653 & 8.99 & 9.63 & 8.26 & 0.515 & 0.031 & 5.6 & 1.0 & 4.5 & 0.8 \\
3409635486731094400 & FO & 3.14835 & 6.23 & 6.75 & 5.59 & 1.428 & 0.061 & 6.6 & 0.9 & 6.1 & 0.8 \\
5334449269746243328 & FO & 3.21183 & 8.42 & 8.81 & 7.89 & 0.425 & 0.032 & 6.5 & 1.4 & 4.9 & 1.1 \\
511226491206912128 & FO & 3.22284 & 9.83 & 10.65 & 8.96 & 0.481 & 0.037 & 5.0 & 1.1 & 3.9 & 0.9 \\
1971722045688053248 & FO & 3.28391 & 8.67 & 9.33 & 7.92 & 0.561 & 0.032 & 7.0 & 1.2 & 5.6 & 1.0 \\
1964855904803120640 & FO & 3.33233 & 5.72 & 6.03 & 5.32 & 1.151 & 0.066 & 7.1 & 1.2 & 6.4 & 1.1 \\
6058439910929477120 & FO & 3.34248 & 5.26 & 5.65 & 4.81 & 1.778 & 0.087 & 5.3 & 0.8 & 4.9 & 0.7 \\
429635993926502912 & FO & 3.65163 & 10.44 & 11.33 & 9.53 & 0.327 & 0.028 & 6.9 & 1.7 & 4.8 & 1.2 \\
5932565900081831040 & FO & 3.78678 & 8.58 & 9.10 & 7.93 & 0.474 & 0.038 & 5.3 & 1.2 & 4.1 & 1.0 \\
5519380077440172672 & FO & 4.22646 & 5.53 & 5.89 & 5.11 & 1.217 & 0.057 & 6.3 & 0.9 & 5.7 & 0.8 \\
428839329030983040 & FO & 4.30649 & 8.68 & 9.37 & 7.90 & 0.509 & 0.030 & 6.5 & 1.1 & 5.1 & 0.9 \\
5881995546318024704 & FO & 4.37292 & 8.65 & 9.30 & 7.92 & 0.463 & 0.038 & 6.8 & 1.6 & 5.2 & 1.2 \\
4514145288240593408 & FO & 4.47115 & 5.11 & 5.59 & 4.57 & 1.810 & 0.107 & 5.7 & 1.0 & 5.3 & 0.9 \\
2004036486267748352 & FO & 5.44565 & 8.09 & 8.63 & 7.41 & 0.496 & 0.038 & 5.5 & 1.2 & 4.3 & 0.9 \\
5506374096132016512 & FO & 5.69296 & 5.44 & 5.85 & 4.96 & 1.261 & 0.064 & 4.9 & 0.8 & 4.5 & 0.7 \\
5337634589276921856 & FO & 5.72548 & 8.82 & 9.39 & 8.13 & 0.355 & 0.029 & 5.4 & 1.3 & 3.9 & 0.9 \\
\hline\hline
\end{tabular}
\end{table*}
